Charge Carrier Dynamics of Methylammonium Lead-Iodide Perovskite Solar Cells

Transient opto-electrical measurements of methylammonium lead iodide (MALI) perovskite solar cells (PSCs) are performed and analyzed in order to elucidate the operating mechanisms. The current response to a light pulse or voltage pulse shows an extraordinarily broad dynamic range covering 9 orders of magnitude in time - from microseconds to minutes - until steady-state is reached. Evidence of a slowly changing charge density at the perovskite layer boundaries is found, which is most probably caused by mobile ions. Current-voltage curves (IV curves) are measured with very fast scan-rate after keeping the cell for several seconds at a constant voltage as proposed by Tress et al. Numerical drift-diffusion simulations reproduce the measured IV curves using different distributions of ions in the model. Analysing the band diagram of the simulation result sheds light on the operating mechanism. To further investigate the effects at short time scales (below milliseconds) photo-generated charge extraction by linearly increasing voltage (photo-CELIV) experiments are performed. We postulate that mobility imbalance in combination with deep hole trapping leads to dynamic doping causing effects from microseconds to milliseconds. Comprehensive transient drift-diffusion simulations of the photo-CELIV experiments strengthen this hypothesis. This advanced characterization approach combining dynamic response measurements and numerical simulations represents a key step on the way to a comprehensive understanding of device working mechanisms in emerging perovskite solar cells.

==> Content/declaration.tex <==



\chapter{Declaration}\label{declaration}


I hereby declare, that I am the sole author and composer of my Thesis and that no other sources or learning aids, other than those listed, have been used. Furthermore, I declare that I have acknowledged the work of others by providing detailed references of said work.
I hereby also declare, that my Thesis has not been prepared for another examination
or assignment, either wholly or excerpts thereof.

\vspace{40mm}

Martin Neukom

\vspace{10mm}

Winterthur, \submissiondate


==> Context/titlePagePrint.tex <==
% Title Page Print

\begin{titlepage}

\begin{addmargin}[-0.3cm]{-3cm} %printversion +1cm %screenversion -1cm
\begin{center}

% Logo University
%\begin{picture}(0,0)															
%\put(-270, -70){\scalebox{0.35}{
%	\includegraphics{images/logos/albert_Ludwigs_university_freiburg_logo.png}
%}}
%\end{picture}

% Logo Fraunhofer ISE
%\begin{picture}(0,0)
%\put(-130, -20){\scalebox{0.2}{
%	\includegraphics{images/logos/fraunhofer_ise_logo.png}
%}}
%\end{picture}

% Logo Fluxim
%\begin{picture}(0,0)																			
%\put(100, 0){ \scalebox{0.13}{
%	\includegraphics{images/logos/fluxim_logo.pdf}
%}}
%\end{picture}



\large

\hfill
\vfill

% Title Picture - Probe Tips
%\scalebox{0.2}{
%\includegraphics{images/title/title_probes.jpg}
%}
%\vspace{5mm}

%\begingroup
%\color{Maroon}\spacedallcaps{\myTitle} \\ \bigskip % Thesis title
%\endgroup
%\spacedlowsmallcaps{\mySubtitle}
%\vfill


Master-Thesis\\
\myName \\
\vspace{5mm}
Albert-Ludwigs-University Freiburg \\
Master Online of Photovoltaics \\
\submissiondate



\end{center}

%\vfill

\end{addmargin}

\end{titlepage}


%% Backside Title  -----------------------------------------
\thispagestyle{empty}
\hfill
\vfill
\noindent\myName: \textit{\myTitle, \mySubtitle, \myYear}
%% Backside Title  -----------------------------------------






